Matching Feature Sets for Few-Shot Image Classification

In image classification, it is common practice to train deep networks to extract a single feature vector per input image. Few-shot classification methods also mostly follow this trend. In this work, we depart from this established direction and instead propose to extract sets of feature vectors for each image. We argue that a set-based representation intrinsically builds a richer representation of images from the base classes, which can subsequently better transfer to the few-shot classes. To do so, we propose to adapt existing feature extractors to instead produce sets of feature vectors from images. Our approach, dubbed SetFeat, embeds shallow self-attention mechanisms inside existing encoder architectures. The attention modules are lightweight, and as such our method results in encoders that have approximately the same number of parameters as their original versions. During training and inference, a set-to-set matching metric is used to perform image classification. The effectiveness of our proposed architecture and metrics is demonstrated via thorough experiments on standard few-shot datasets -- namely miniImageNet, tieredImageNet, and CUB -- in both the 1- and 5-shot scenarios. In all cases but one, our method outperforms the state-of-the-art.

==> algorithm_pretrain.tex <==
\begin{algorithm}[t]
    \SetAlgoLined
    {\small
        \KwData{
        SeatFeat (SF$_{\textrm{epoch}}$) of the epoch with four level convolution $f(\cdot| \{ \theta^{f}_{l}\}_{l=1}^4$) and
        set of mappers $\{\{g_{l, j}(\mathbf{z}_l|{\theta^{g}_{l, j}})\}_{j=1}^{l}\}_{l=1}^4$,
        fully connected heads $o_{l, j}$, maximum epoch Max$_e$, number of classes  $N_b$, cross-entropy criterion($\cdot, \cdot$), batch based train $\mathcal{D}^{\text{train}}$ and validation $\mathcal{D}^{\text{valid}}$ datasets, and episodic error function $E(\cdot|\mathcal{D})$ using eq.~\ref{eq:inference}.
        }  
        \KwResult{best validated SeatFeat model SF$_{\textrm{best}}$
        % $g(\cdot|{\theta^{g}_\textrm{best}})$ 
        % $\{\{g_{l, j}(\mathbf{z}_l|{\theta^{g}_{\textrm{best}, l, j}})\}_{j=1}^{l}\}_{l=1}^4$
        }   
        \For{\text{epoch} $\in \{1,\ldots,\text{max}_e\}$}{   
        % {\color{teal}  \# training loop}    \ \\
        \For{$(\mathbf{x}, y) \in \mathcal{D}^\text{train}$} {   
        $m \leftarrow 0$; 
        $\text{logits} \leftarrow []$; 
        $y^\prime \leftarrow []$ \\
            \For{$b\in\{1,B\}$} {
            $\mathbf{z}_b \leftarrow f(\mathbf{x}|\{\theta^f_i\}_{i=1}^b)$ \ \\ 
                \For{$j\in\{1,\ldots,i\}$} { 
                    $\mathbf{h}_{l, j} \leftarrow g_{b,j}(\mathbf{z}_b|{\theta^{g}_{b,j}})$; \\
                    $\text{logits} \leftarrow [\text{logits}, o_{l,j}(\mathbf{h}_{b,j}))]$ \\
                    $y^\prime \leftarrow [y^\prime, y+(N_b \times m)]$ \\
                    $m \leftarrow m + 1$
                } 
            } 
        $\text{loss} \leftarrow \text{criterion}(\text{logits}, y^\prime)$ \ \\
        loss backpropagation and parameter update  {\color{teal}  \# sgd}  \ \\  
        }  
         
        \textbf{if} \ {$E(\text{SF}_\text{epoch} | \mathcal{D}^{\text{valid}}) < E( \textrm{SF}_{\textrm{best}} | \mathcal{D}^{\text{valid}})$}: {\color{teal}  \# validation } \ \\
         \quad \quad  $\textrm{SF}_{\textrm{best}} \leftarrow \textrm{SF}_\textrm{epoch}$ \ \ \ \quad \quad {\color{teal}  \# update the best model }
        } 
    }
    \caption{SetFeat pre-training and validation.}
    \label{algo:pretraining}
\end{algorithm} 




 
 

==> table_numofParameters.tex <==
\begin{table}[hbt!]
\centering
\caption{number of parameters in the original feature extractor and {\color{blue}our} set feature extractor.} 
    \begin{tabular}{rcc}   
       \toprule
        & backbone     & \# of params. \\ 
        \midrule
        & Conv4-64                          & 0.113 M   \\  
         & {\color{blue}SetFeat4-512}        & 0.238 M  \\[0.5em]
          & Conv4-512                       & 1.591 M  \\  
         & {\color{blue}SetFeat4-512}        & 1.583 M  \\[0.5em]
         
         &ResNet18                             & 11.511 M  \\  
         &{\color{blue}SetFeat12$^{*}$}       & 11.466 M  \\[0.5em]
         
         &ResNet12                            & 12.424 M  \\  
         &{\color{blue}SetFeat12}             & 12.349 M  \\[0.5em]  
         
        \bottomrule
    \end{tabular}
    \\ 
    \label{tab:margin_ablation}
\end{table}


